GENOT: Entropic (Gromov) Wasserstein Flow Matching with Applications to Single-Cell Genomics

Single-cell genomics has significantly advanced our understanding of cellular behavior, catalyzing innovations in treatments and precision medicine. However, single-cell sequencing technologies are inherently destructive and can only measure a limited array of data modalities simultaneously. This limitation underscores the need for new methods capable of realigning cells. Optimal transport (OT) has emerged as a potent solution, but traditional discrete solvers are hampered by scalability, privacy, and out-of-sample estimation issues. These challenges have spurred the development of neural network-based solvers, known as neural OT solvers, that parameterize OT maps. Yet, these models often lack the flexibility needed for broader life science applications. To address these deficiencies, our approach learns stochastic maps (i.e. transport plans), allows for any cost function, relaxes mass conservation constraints and integrates quadratic solvers to tackle the complex challenges posed by the (Fused) Gromov-Wasserstein problem. Utilizing flow matching as a backbone, our method offers a flexible and effective framework. We demonstrate its versatility and robustness through applications in cell development studies, cellular drug response modeling, and cross-modality cell translation, illustrating significant potential for enhancing therapeutic strategies.

==> chapters/0_abstract.tex <==
Latent linear interpolations are a powerful tool to navigate the representation space of deep generative models. This aspect is particularly relevant in applied settings, where meaningful latent traversals can be learnt to represent the evolution of a system's trajectory and mapped back to the data space. However, when data lies on manifold with complex geometry, linear interpolations of the representation space do not directly correspond to geodesic paths along the manifold unless enforced. An example of such a setting is scRNA-seq, where high-dimensional and discrete cellular data is assumed to lie on a Negative Binomial statistical manifold modelled by the decoder of a Variational Autoencoder. In this work, we introduce \textsc{FlatVI}, a novel training framework enforcing Euclidean geometry in the latent space of discrete-likelihood Variational Autoencoders modelling count data. We showcase our model for learning latent trajectories on discrete single-cell RNA-seq data in combination with Euclidean optimal transport. Results on four temporally-resolved biological datasets, ranging from development to infection, demonstrate that our framework improves the reconstruction of cell state evolution, as well as the learning of biologically meaningful velocity fields.

%The assumption of a Euclidean representation space of single-cell transcriptomics has proved powerful in unveiling cellular processes in multiple applications, such as modelling cellular trajectories and response s to drugs. Among the various methods leveraging Euclidean geometry, Optimal Transport stands out as a flexible tool in single-cell analysis. Yet, most of the existing deep representation learning techniques for single-cell data are prone to induce non-linear geometries. We lift the linearity concern by introducing FlatVI, a novel approach to incorporate the geometry of the data into single-cell representations, enhancing the application of Optimal Transport. We achieve this by implementing a ``flattening'' regularisation for discrete-likelihood Variational Autoencoders aligning the latent space with Euclidean structure and accounting for critical data characteristics such as sparsity and geometry. Results on four temporally-resolved biological datasets, ranging from development to infection, demonstrate that these constraints improve the reconstruction of latent trajectories as well as the learning of biologically meaningful velocity fields.


==> chapters/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
Generative models for representation learning like Variational Autoencoders (VAEs) have influenced computational sciences in multiple scientific domains \cite{albergo2023building}. One reason is that real-world experimental data often poses significant modelling challenges as it is inherently noisy, high-dimensional, and complex \textbf{CITE}. As a solution, learning a low-dimensional and dense latent representation of the data has gained traction in applied machine learning. One example is learning population dynamics in high-dimensional systems, where modelling interpolations in a well-behaved low-dimensional data embedding can offer valuable insight into the system's evolution through time \textbf{CITE}. Furthermore, with the decoder parameterising a flexible likelihood model, VAEs present a promising avenue for representing both continuous and discrete data. The latter setting has shown unprecedented potential on cellular data, in particular gene expression, which is collected via single-cell RNA-seq (scRNA-seq) \textbf{CITE}, measuring thousands of genes in parallel.  The resulting discrete vectors describe the state of a cellular system across diverse biological settings \textbf{CITE}.

The connection between VAEs and Riemannian geometry justifies operating in the VAE's latent space, where the latent codes parameterise a low-dimensional representation of the data manifold \textbf{CITE}. This is especially relevant in the setting of population dynamics, where popular approaches still assume Euclidean geometry in the representation space \textbf{CITE}. A notable example is the standard formulation of dynamic Optimal Transport (OT) \textbf{CITE}, which exploits straight-line interpolations between observations to learn a time-dependent map across population snapshots. \emph{However, building latent trajectories upon the Euclidean assumption is sub-optimal when the data lies on a non-Euclidean manifold}, as straight lines do not reflect geodesic paths on complex geometries (see \cref{fig:concep_figure}). While methods exist to endow the latent representation of a VAE with Euclidean geometry \textbf{CITE}, the scope of existing work revolves around continuous data, neglecting the discrete domain. 
In particular, no prior work has extended existing frameworks for learning latent geodesic trajectories to statistical manifolds of discrete probability distributions.

In this work, we close this research gap and introduce FlatVI, Flat Variational Inference, a simple and theoretically principled approach to ensure the correspondence between straight latent paths and geodesic paths along the data manifold. Our focus on statistical manifolds---those manifolds whose points correspond to probability distributions of a pre-defined family, defined over the corresponding parameter space $\mathcal{H}$---enables us to draw connections to the theory of VAEs. When trained as a likelihood model, a VAE's decoder image matches the manifold's parameter space $\mathcal{H}$. This formulation finds direct application in scRNA-seq, where individual gene counts are assumed to follow a negative binomial distribution, reflecting crucial data properties such as discreteness and overdispersion \textbf{CITE}.



% Points on statistical manifolds correspond to probability distributions of a pre-defined family and are defined over the corresponding parameter space $\mathcal{H}$ \textbf{CITE}. Such manifolds are essential for modelling data that follows a particular noise model. Moreover, they are intrinsically connected to VAEs, as the decoder of a VAE, trained as a likelihood model, spans the parameter space $\mathcal{H}$. This formulation finds direct application in scRNA-seq, where individual gene counts are assumed to follow a negative binomial distribution, reflecting crucial data properties such as discreteness and overdispersion \textbf{CITE}.

% In this study, we introduce \textsc{FlatVI} (Flat Variational Inference), a simple and theoretically principled approach to enforce Euclidean geometry in the latent space of discrete-likelihood VAEs, while maintaining correspondence between straight latent paths and geodesic paths along the data manifold. 
Crucially, FlatVI achieves this correspondence through a \textit{flattening loss} that pushes the pullback metric from a stochastic VAE decoder towards spatially-uniform scaled identity matrix, thus reflecting latent Euclidean geometry (\cref{fig:concep_figure}). Our method finds direct applications to single-cell representation learning and trajectory inference, which we demonstrate across multiple biological settings by providing an improved data representation for OT-based modelling of latent cellular population dynamics. 

In summary, we make the following contributions:
\begin{enumerate}
    \item We introduce a regularisation technique for discrete-likelihood VAEs to enforce correspondence between straight latent interpolations and geodesic paths on the statistical manifold spanned by the decoder.
    \item We provide an explicit formulation of the flattening loss for the negative binomial case, which directly impacts modelling high-dimensional scRNA-seq data. 
    \item We show that our method offers a better representation space for existing OT-based trajectory inference tools than existing approaches.
\end{enumerate}


==> chapters/2_related_work.tex <==
\todo{Geometry in single-cell}
\section{Related work}\label{sec: related_works}
% ====FIGURE============
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/model_fig.png} % Replace 'example-imawige' with the filename of your image
    \caption{Visual conceptualisation of the proposed latent space flattening approach for single-cell VAEs by regularising the pullback metric of a statistical manifold. OT trajectories are learnt in the flat latent space endowed with Euclidean geometry.}
    \label{fig:concep_figure}
\end{figure*}
%
We continue to discuss related work on geometry-aware representation learning as well as OT methods for modelling gene expression and trajectories.
% The following paragraphs contextualise the FlatVI model within the scope of said fields.
%
\vspace{-0.4em}
\paragraph{Geometry-regularised AEs} Using latent variable models to learn representations of scRNA-seq data is well established \citep{Lopez2018, Eraslan2019}. Yet, enforcing a specific geometric structure in the learnt latent spaces is less explored in this context. \citet{geometrically_enriched} modelled optimal latent paths reflecting the geometry of the observation space defined by both deterministic and Gaussian stochastic decoders. Successively, \citet{arvanitidis2022pulling} extended the approximation of geodesic latent paths to VAEs with arbitrary likelihood. While these works leverage the geometry of the observation space to learn latent interpolations along the data manifold, \citet{chen2020learning} explored the benefits of representation learning when modelling the latent space of deterministic AEs as flat manifolds. Other works incorporate data geometry into the latent space of AE models through isometric  \citep{lee2022regularized} and Jacobian \citep{nazari2023geometric} regularisations. 
%In this work, we extend prior work by assuming the observation space to be a statistical manifold whose geometry is governed by the Fisher rather than the Euclidean metric. 
%
\vspace{-0.4em}
\paragraph{OT for single-cell genomics} OT methods in single-cell transcriptomics have shown potential in multiple application contexts, such as trajectory inference \citep{Schiebinger2019, lange2022moslin}, spatial reconstruction \citep{Moriel2021} and multi-modal alignment \citep{demetci2022scot}. Recent efforts have resorted to predicting the effects of drug perturbations on cells \citep{hetzel2022predicting} using neural OT \citep{Bunne2023} and cell trajectories in an unbalanced setting \citep{eyring2022modeling}. The works from \citet{Tong2020TrajectoryNet} and \citet{mioflow} explore the applicability of OT for modelling gene expression through time. \citet{mioflow} model continuous single-cell trajectories in a latent space where distances are regularised to approximate the geodesic distances of single-cell data. 
% This regularisation, however, does not incorporate the distributional properties of RNA-seq measurements such as sparsity or overdispersion. 
% In contrast, our method explicitly considers such characteristics by modelling trajectories on a Negative Binomial manifold. 
% Our work revolves around modelling gene expression through time via continuous OT \citep{peyré2020computational}
%
% \vspace{-0.4em}
% \paragraph{Flow-based OT} Modelling continuous trajectories via Continuous Normalizing Flows (CNF) has been explored in the field of single-cell genomics \citep{Tong2020TrajectoryNet, mioflow, Klein2023}. Recently, novel approaches based on Flow Matching \citep{lipman2023flow} have provided a faster and more stable training scheme by introducing simulation-free objectives to learn the CNF vector field \citep{liu2022flow, pooladian2023multisample, albergo2023building}. Leveraging such tractable formulations of flows and establishing a connection to OT, CFM was successfully applied to trajectory inference \citep{tong2023, neklyudov2023action}. Further, \citet{chen2023riemannian} introduced a geometrically informed version of CFM. 

% In the context of CFM, our work is most similar to the concept of geometrically informed Flow Matching discussed by \citet{chen2023riemannian}.

% position our work in 1-2 sentences building on the related work 
Here, we extend prior work on geometry-informed AEs by modelling the correspondence between Euclidean latent space and the statistical manifold of the single-cell observation space, whose geometry is governed by the Fisher Information metric. This aspect enables us to explicitly deal with the distributional characteristics of single-cell data. Being able to account for properties such as sparsity or overdispersion in a rigorous manner is a key difference distinguishing our work from \citet{mioflow} (see \cref{sec: comparison_huguet} for more details about the comparison).
% Due to is geoOur works is most As we are also using CFM to model trajectories, our work is similar in spirit to the geometrically informed version of CFM by \citet{chen2023riemannian}.

==> chapters/3_method.tex <==
\section{Background}
Following the structure of the related works in \cref{sec: related_works}, we move on to present the theoretical background required for our FlatVI model, cf. \cref{sec:flatvi}.
%
\subsection{VAEs for discrete data}\label{sec: sc_vae}
In this work, we deal with discrete count data, formally collected in a high-dimensional matrix $\mathbf{X} \in \mathbb{N}_0^{N \times G}$, where $N$ represents the number of observations and $G$ the number of features. We assume that individual sample features $\mathbf{x}_{ng}$ are independent realisations of a discrete random variable $\mathbf{X}_{ng}\sim\mathbb{P}(\phi_{ng})$ with observation-specific parameters $\phi_{ng}$. \looseness=-1

Let $\mathbf{x}\in \mathcal{X}$ be an observation. We consider a joint latent variable model factorising as follows:
%
\begin{equation}
p_\phi(\mathbf{x},\mathbf{z})=p_\phi(\mathbf{x}|\mathbf{z})p(\mathbf{z})\; ,\nonumber
\end{equation}
%
where $\mathbf{z}$ is a $d$-dimensional latent random variable with $d<G$ and $\mathbf{z} \sim p(\mathbf{z})$ with $p(\mathbf{z})=\mathcal{N}(\mathbf{0}, \mathbb{I}_d)$. In other words, the latent variable $\mathbf{z}\in \mathcal{Z}$ is sampled from a known prior distribution, while the observation model is a discrete distribution from a pre-defined family with parameters expressed as a function of the latent variable $\mathbf{z}$ as:
%
\begin{equation}
p_\phi(\mathbf{x}|\mathbf{z}) = \mathbb{P}(\mathbf{x}|h_\phi(\mathbf{z})) \; ,
\end{equation}
%
In deep latent variable models, $h_\phi$ is a deep neural network termed \textit{decoder}. VAEs additionally add an \textit{encoder} network $f_\psi: \mathcal{X}\to\mathcal{Z}$ optimised jointly with $h_\phi$ through the Evidence Lower Bound (ELBO) objective, which introduces the following loss: 
%
\begin{align}
\label{elbo}
\mathcal{L}_\textrm{ELBO} =  \mathbb{E}_{q_\psi(\mathbf{z} \mid \mathbf{x})}\big[\log p_\phi(\mathbf{x} |h_\phi(\mathbf{z}))\big]
 - \textrm{KL}\big(q_\psi(\mathbf{z} | \mathbf{x}) \lVert p(\mathbf{z})\big)\: ,
\end{align}
%
where the first term denotes the likelihood of the data under the decoder model and the second term is the Kullback-Leibler divergence between a Gaussian variational posterior distribution parameterised by $f_\psi$ and a standard multivariate Gaussian prior \cite{kingma2022autoencoding}. In other words, as long one can select a reasonable family of distributions $\{\mathbb{P}(\cdot|\phi)\}_{\phi \in \mathcal{H}}$, the data can be modelled with a VAE.

In the field of scRNA-seq biological and technical variability causes an inherent overdispersion of the expression counts, making the negative binomial likelihood a natural choice for modelling gene expression \citep{Heumos2023}. Thus, we assume $\mathbb{P}(\phi_{ng})=\mathrm{NB}(\mu_{ng}, \theta_g)$, where $\mu_{ng}$ and $\theta$ represent the cell-gene-specific mean and the gene-specific inverse dispersion parameters, respectively. In the VAE setting, given a gene-expression vector $\mathbf{x}$, we define the following parametrisations:
%
\begin{align}
    \mathbf{z} & = f_{\psi}(\mathbf{x}), \\
    \bm{\mu} & =  h_{\phi} \label{eq: decoder}(\mathbf{z}, l) = l \: \textrm{softmax}(\rho_{\phi}(\mathbf{z})) \: , 
\end{align}
where $\rho_{\bm{\phi}}: \mathbb{R}^d \to \mathbb{R}^G$ models expression proportions of individual genes and $l$ is the observed cell-specific size factor directly derived from the data as a cell's total number of counts $l=\sum_{g=1}^G\mathbf{x}_{g}$. The encoder $f_{\bm{\psi}}$ already takes into account the reparametrisation trick \citep{kingma2022autoencoding}. In what follows, we drop the dependency of $h$ on $\phi$ for notational simplicity.


\subsection{The geometry of autoencoders}
\paragraph{Deterministic Autoencoders.} A common assumption is that continuous data lies near a low-dimensional Riemannian manifold $\mathcal{M}_\sX$ associated with a latent representation $\mathcal{Z}$ and with $\mathcal{X}=\mathbb{R}^G$. The decoder of a deterministic AE model can be seen as an immersion $h:\mathbb{R}^d \rightarrow\mathbb{R}^G$ of the latent space $\mathcal{Z} = \mathbb{R}^d$ into the embedded Riemannian manifold $\mathcal{M}_{\sX}$ equipped with a metric tensor $\mathrm{M}$ defining the local geometry of the manifold \citep{geometrically_enriched}. 
%
\begin{definition}\label{def: riem_manif}
    A Riemannian manifold is a smooth manifold $\mathcal{M}_{\sX}$ endowed with a Riemannian metric $\mathrm{M}(\mathbf{x})$ for $\mathbf{x}\in\mathcal{M}_{\sX}$. $\mathrm{M}(\mathbf{x})$ is a positive-definite matrix that changes smoothly and defines a local inner product on the tangent space $\mathcal{T}_\mathbf{x}\mathcal{M}_{\sX}$ as the equation $\langle\mathbf{u}, \mathbf{v}\rangle_{\mathcal{M}_\mathcal{X}} = \mathbf{u}^\mathbf{T}\mathrm{M}(\mathbf{x})\mathbf{v}$, with $\mathbf{v}, \mathbf{u} \in \mathcal{T}_\mathbf{x}\mathcal{M}_{\mathbf{x}}$ \citep{geometrically_enriched}.
\end{definition}
%
From \cref{def: riem_manif}, it derives that a Riemaniann manifold has Euclidean geometry if $\mathrm{M}(\mathbf{x})=\mathbb{I}_G$ everywhere.

In this setting, the geometry of the latent space is directly linked to that of observation space through the \textit{pullback metric} \citep{arvanitidis2022pulling}
%
\begin{equation}\label{eq: pullback_metric}
    \mathrm{M}(\mathbf{z}) = \mathbb{J}_h(\mathbf{z})^\textrm{T}\mathrm{M}(\mathbf{x})\mathbb{J}_h(\mathbf{z})\: , 
\end{equation}
%
where $\mathbf{x}=h(\mathbf{z})$ and $\mathbb{J}_h(\mathbf{z})$ is the Jacobian matrix of $h(\mathbf{z})$. As such, we identify a latent Riemanniann manifold $\mathcal{M}_\mathbf{z}$, whose properties are defined based on the geometry of $\mathcal{M}_{\sX}$ through \cref{eq: pullback_metric}. For example, \cref{eq: pullback_metric} allows to define the shortest curve $\gamma(t)$ connecting pairs of latent codes $\mathbf{z}_1$ and $\mathbf{z}_2$ as the one minimising the distance between their images $h(\mathbf{z}_1)$ and $h(\mathbf{z}_2)$ on $\mathcal{M}_\mathcal{X}$. More formally:
%
\begin{align} \label{dist}
d_{\textrm{latent}}(\mathbf{z}_1,\mathbf{z}_2)&=\inf_{\gamma(t)}\int_0^1\lVert \dot{h}(\gamma(t)) \rVert \d t =\inf_{\gamma(t)}\int_0^1\sqrt{\dot{\gamma}(t)^\textrm{T}\mathrm{M}(\gamma(t))\dot{\gamma}(t)} \d t \; , \\ 
\mathrm{where} \quad &\gamma(0)=\mathbf{z}_1,\ \gamma(1)=\mathbf{z}_2 \: . \nonumber
\end{align}
%
Here, $\gamma(t): \mathbb{R} \rightarrow \mathcal{Z}$ is a curve in the latent space with boundary conditions $\gamma(0)=\mathbf{z}_1$ and $\gamma(1)=\mathbf{z}_2$, and $\dot{\gamma}(t)$ its derivative along the manifold. Crucial to this work, one notices that combining  \cref{dist} and \cref{def: riem_manif},\textit{ when the the metric tensor $\mathrm{M}(\mathbf{z})=\mathbb{I}_d$, the curve $\gamma^*(t)$ minimising \cref{dist} is the straight line between latent codes}.

\paragraph{Variational Autoencoder.} While in AE one deals with deterministic manifolds, in VAEs the decoder function $h$ maps a latent code $\mathbf{z} \in \mathcal{Z}$ to the parameter configuration $\bm{\mu} \in \mathcal{H}$ of the data likelihood, where $\mathcal{H}=\mathbb{R}^G$ represents the parameter space. As such, the decoder image lies on a statistical manifold, which is a smooth manifold of probability distributions. Such manifolds have a natural metric tensor called \textit{Fisher Information Metric }(FIM) \citep{frankinfgeom,arvanitidis2022pulling}. The FIM defines the local geometry of the statistical manifold and can be used to build the pullback metric for arbitrary decoders. For a statistical manifold $\mathcal{M}_{\mathcal{H}}$ with parameters $\bm{\mu}\in\mathcal{H}$, the FIM is formulated as
%
\begin{equation}\label{eq: fisher_info_decoder}
    \mathrm{M}(\bm{\mu}) = \mathbb{E}_{p(\mathbf{x}\mid\bm{\mu})} \left[\nabla_{\bm{\mu}}\log p(\mathbf{x} \mid \bm{\mu}) \nabla_{\bm{\mu}}\log p(\mathbf{x} \mid \bm{\mu})^\textrm{T} \right]\: , 
\end{equation}
%
where $\bm{\mu}=h(\mathbf{z})$ and the metric tensor $\mathrm{M}(\bm{\mu})\in \mathbb{R}^{G \times G}$ \citep{arvanitidis2022pulling}. Analogous to deterministic AEs, one can combine \cref{eq: fisher_info_decoder} and \cref{eq: pullback_metric} to formulate the pullback metric for an arbitrary statistical manifold, with the difference that the pulled-back metric tensor is defined in $\mathcal{H}$. As a result, the latent space of a VAE is endowed with the pullback metric for a statistical manifold
%    
\begin{equation}\label{eq: pullback_info_geom}
    \mathrm{M}(\mathbf{z}) = \mathbb{J}_h(\mathbf{z})^\textrm{T}\mathrm{M}(\bm{\mu})\mathbb{J}_h(\mathbf{z}) \: ,
\end{equation}
%
where $\mathrm{M(\mathbf{z})} \in \mathbb{R}^{d \times d}$. Note that the calculation of the FIM is specific for the chosen likelihood type and, as such, depends on initial assumptions on the data distribution. 

\subsection{Learning population dynamics with optimal transport}
The complexity of learning trajectories in high-dimensional data can be obviated by \textit{interpolating latent representations and decoding intermediate results to the data space for inspection}. In the imaging domain \textbf{CITE} or even drug discovery \textbf{CITE} this has been achieved by performing linear interpolation or latent space arithmetics. Here, we are concerned with learning population dynamics which consists of modelling the temporal evolution of a dynamical system from unpaired samples of observations through time. As such a task can be seen as a distribution matching problem, dynamic optimal transport (OT) has been a popular avenue for tackling population dynamics. 

OT computes the most efficient mapping for transporting mass from one measure, $\nu$, to another $\eta$, defined on $\mathcal{Y}$. Relevant to dynamical systems, \citet{Benamou2000} introduced a \emph{continuous formulation} of the OT problem. In this setting, let $p_t$ be a time-varying density over $\mathbb{R}^d$ constrained by $p_0=\nu$ and $p_1=\eta$. Dynamic OT learns a time-dependent vector field $u: [0,1] \times \mathbb{R}^d \to \mathbb{R}^d$ minimising the Wasserstein-2 distance:
%
\begin{equation}\label{eq: dynamic_wasserstein}
W_2(\nu, \eta)^2 = \inf_{p_t, u_t} \int_{0}^{1}\int_{\real{d}}\norm{u_t(\mathbf{x})}^2 p_t(\mathbf{x}) \,\d\mathbf{x}\,\d t\: , 
\end{equation}
%
where $u_t(\mathbf{x})=u(t,\mathbf{x})$. The velocity field $u_t(\mathbf{x})$ is associated with an ordinary differential equation (ODE) $\textrm{d}\mathbf{x} = u_t(\mathbf{x})\textrm{d} t$ whose solution is an integration map that matches a source with a target distribution. Therefore, one can use dynamic OT to learn a system's dynamics from snapshots of data collected over time. Notably, the norm of the vector field in \cref{eq: dynamic_wasserstein} assumes Euclidean geometry.  

An efficient formulation of dynamic OT comes from  \citet{tong2023}, who demonstrated that the time-resolved marginal vector field $u_t(\mathbf{x})$ has the same minimiser as the conditional vector field $u_t(\mathbf{x}|\mathbf{x}_0,\mathbf{x}_1)$, where $(\mathbf{x}_0, \mathbf{x}_1)\sim\pi(\mathbf{X}_0, \mathbf{X}_1)$ are tuples of points sampled from the static OT coupling of batches source and target batches, $\mathbf{X}_0$ and $\mathbf{X}_1)$. Assuming Gaussian marginals $p_t$ and $\mathbf{x}_0$ and $\mathbf{x}_1$ to be connected by Gaussian flows, both $p_t(\mathbf{x} \mid \mathbf{c})$ and $u_t(\mathbf{x} \,|\, \mathbf{c})$ become tractable:
%
\begin{equation}\label{eq: marginal_p}
p_t(\mathbf{x} \,|\, \mathbf{c}) = \mathcal{N}(t\mathbf{x}_1 + (1-t)\mathbf{x}_0, \sigma^2)
\end{equation}
%
\begin{equation}\label{eq: cfm_vf}
u_t(\mathbf{x} \,|\, \mathbf{c}) = \mathbf{x}_1 - \mathbf{x}_0 \: ,
\end{equation}
%
with a pre-defined value of $\sigma^2$. Accordingly, the OT-CFM loss is
%
\begin{equation}\label{eq: cfm_loss}
\mathcal{L}_{\textrm{OT-CFM}} = \mathbb{E}_{t, q(\mathbf{c}), p_t(\mathbf{x} \mid \mathbf{c})}\big [ \lVert  v_\xi(t,\mathbf{x})-u_t(\mathbf{x} \mid  \mathbf{c})\lVert^2 \big ] \: ,
\end{equation}
%
with $t\sim\mathcal{U}(0,1)$. From \cref{eq: dynamic_wasserstein} and \cref{eq: marginal_p}, one can highlight three aspects:
\begin{enumerate}
    \item One cannot apply Dynamic OT directly to discrete state spaces.
    \item OT-CFM benefits from low-dimensional representations since the OT-coupling is optimised based on distances in the state space.
    \item OT-CFM uses straight lines to optimise the conditional vector field, thus assuming Euclidean geometry.
\end{enumerate}
%
As discussed, one can tackle (1) and (2) by learning dynamics in a low-dimensional representation of the state space--the latent space of a VAE with discrete-likelihood decoder. Note, however, that (3) is still a shortcoming, since straight lines in the latent space of a VAE do not reflect geodesic paths a the data manifold unless enforced otherwise. We tackle this challenge by applying OT-CFM to the latent space of a VAE with enforced Euclidean geometry.

\section{The FlatVI model}
\label{sec:flatvi}
%
After outlining our approach to OT-based trajectory inference, we introduce FlatVI, a method to align Euclidean latent space with the NB manifold of VAEs to enhance single-cell OT.
%
\vspace{-0.4em}
\paragraph{Problem setting}
For time-resolved scRNA-seq data, cells are collected in $T$ unpaired distributions $\{\nu_t\}_{t=0}^T$. Individual time points correspond to separate snapshot datasets $\{\mathbf{X}_t\}_{t=0}^T$, each with $N_t$ observations. Every snapshot is mapped to tuples $\{(\mathbf{Z}_t , \mathbf{l}_t)\}_{t=0}^T$ of latent representations $\mathbf{Z}_t\in\mathbb{R}^{N_t \times d}$ and size factors $\mathbf{l}_t \in \mathbb{N}_0^{N_t}$ following the setting described in \cref{sec: sc_vae}. We wish to learn the dynamics of the system through a parameterised function in the latent space $\mathcal{Z}$ of a VAE, taking advantage of its continuity and lower dimensionality properties. 
%
% \vspace{-0.4em}
% \paragraph{Size factor treatment}
% Since the size factors $\mathbf{l}_t$ required for decoding are observed variables derived from single-cell counts in the dataset, their values are not available when simulating novel cell trajectories from $t=0$, hindering the use of the decoder to recover individual gene evolution. Assuming that the size factor is a real number and related to the cell state, we include $\log l_t$ in the latent dynamics and infer its trajectory together with the latent state representation $\mathbf{z}_t$. The $\log$ is taken for training stability. Therefore, we learn a velocity field $v_\xi: [0,1] \times \mathbb{R}^{d+1} \to \mathbb{R}^{d+1}$ on the concatenated state $\mathbf{s}_t=[\mathbf{z}_t, \log l_t]$. The time-resolved vector field $v_\xi$ is modelled by matching subsequent pairs of cell distributions.
% %
% \vspace{-0.4em}
% \paragraph{Gene expression trajectories} If the latent space $\mathcal{Z}$ can be injectively mapped to the parameter manifold $\mathcal{H}$, trajectories in $\mathcal{Z}$ correspond to walks across the continuous parameter space via the stochastic decoder $h$. The temporal trajectory of the likelihood parameter vector $\bm{\mu}_t$ is given by 
% %
% \begin{equation}
%         \bm{\mu}_t = h \left( \mathbf{s}_0 +\int_0^t v_\xi(t', \mathbf{s}_{t'}) \, \textrm{d}t' \right)\: ,
% \end{equation}
% %
% where $\bm{\mu}_0=h(\mathbf{s}_0)$ and we express the decoder function $h(\mathbf{z}_t, l_t)$ from \cref{eq: decoder} as $h(\mathbf{s}_t)$ for simplicity. Then, assuming a gene-wise constant inverse dispersion $\bm{\theta}_g$, discrete trajectories of gene counts follow the noise model $\mathbf{x}_t \sim \textrm{NB}(\bm{\mu}_t, \bm{\theta})$.


% ====FIGURE============
\subsection{Geometry on NB statistical manifolds}
As outlined in \cref{sec: sc_vae}, single-cell counts are modelled with an NB decoder with the following univariate density for each gene $g$ independently:
%
% \begin{align}
% p_{\textrm{NB}}(\mathbf{x}_g \mid &\bm{\mu}_g, \bm{\theta}_g)=\\&\frac{\Gamma(\bm{\theta}_g+\mathbf{x}_g)}{\mathbf{x}_g!\Gamma(\bm{\theta}_g)}\Big(\frac{\bm{\theta}_g}{\bm{\theta}_g+\bm{\mu}_g}\Big)^{\bm{\theta}_g}\Big(\frac{\bm{\mu}_g}{\bm{\theta}_g+\bm{\mu}_g}\Big)^{\mathbf{x}_g}\: ,
% \end{align}
\begin{align}
p_{\textrm{NB}}(\mathbf{x}_g \mid \bm{\mu}_g, \bm{\theta}_g)&=C\: \Big(\frac{\bm{\theta}_g}{\bm{\theta}_g+\bm{\mu}_g}\Big)^{\bm{\theta}_g}\Big(\frac{\bm{\mu}_g}{\bm{\theta}_g+\bm{\mu}_g}\Big)^{\mathbf{x}_g}\: ,\\
&\textrm{where } C = \frac{\Gamma(\bm{\theta}_g+\mathbf{x}_g)}{\mathbf{x}_g!\Gamma(\bm{\theta}_g)} \notag
\end{align}
%
with $\mathbf{x}_g\in \mathbb{N}_0$ and $\bm{\mu}_g=h_g(\mathbf{z})$. Notably, since the decoder $h$ produces cell-specific means, each cell is deemed as an individual probability distribution. Consequently, we assume that the data lies on an embedded NB statistical manifold. According to \cref{eq: pullback_info_geom}, we pull back the FIM of the statistical manifold of the NB probability distribution to the latent space $\mathcal{Z}$.
%
\begin{proposition}
The pullback metric evaluated at the latent point $\mathbf{z} \in \mathcal{Z}$ of a NB statistical manifold parameterised by the mean decoder $h$ and inverse dispersion $\bm{\theta}$ is 
%
\label{prop:fisher_negative_binomial}
\begin{equation} \label{nb_metric}
\mathrm{M}(\mathbf{z})=\sum_g \frac{\bm{\theta}_g}{h_g(\mathbf{z})(h_g(\mathbf{z})+\bm{\theta}_g)}\nabla_\mathbf{z}h_g(\mathbf{z})\otimes\nabla_\mathbf{z}h_g(\mathbf{z}) \: ,
\end{equation}
%
where $\otimes$ is the outer product of vectors and $g$ indexes individual genes.
\end{proposition}
\vspace{-0.5em}
%
\cref{app: derivation_fisher} includes more details about the proof of \cref{prop:fisher_negative_binomial}. Note that we only take the gradient of the decoder, modelling the mean with respect to the latent space, since the inverse dispersion parameter is not a function of the latent space. Having defined $\mathrm{M}(\mathbf{z})$, the distance between latent representations can be computed optimally with respect to the distribution distance between the associated count vectors combining \cref{dist} and \cref{prop:fisher_negative_binomial}.
%
% ==========================================================================================================================================================

\begin{table*}[t]
\centering
\caption{VoR, MF and Negative Log-Likelihood (NLL) as functions of the flattening regularising scale $\lambda$ evaluated on a 10-dimensional latent space. Missing entries indicate diverged values.}
\label{tab:tradeoff_lik_flatness}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\hline
                     & \multicolumn{3}{c|}{EB}   & \multicolumn{3}{c|}{CMV} & \multicolumn{3}{c|}{MEF} & \multicolumn{3}{c}{Pancreas} \\
                     & VoR (\textdownarrow)  & MF (\textdownarrow)      & NLL (\textdownarrow)   & VoR (\textdownarrow)    & MF (\textdownarrow)      & NLL (\textdownarrow)     & VoR (\textdownarrow)      & MF (\textdownarrow)         & NLL (\textdownarrow)     & VoR (\textdownarrow)   & MF (\textdownarrow)      & NLL (\textdownarrow)     \\ \hline
NB-VAE               & 72.1 & -        & 495.1 & 28.5   & -        & 904.0   & 120.2    & -          & 509.0   & 47.3  & -        & 1201.2  \\
FlatVI $\lambda=0.1$ & 62.3 & 19231.4 & 519.5 & 21.3   & 3553.7  & 1006.2  & 13.3     & 1412.6    & 544.3   & 22.2  & 1339.2  & 1239.8  \\
FlatVI $\lambda=1$   & 48.8 & 324.1   & 525.2 & 6.4    & 52.9    & 1072.2  & 21.9     & 120.5     & 553.0   & 15.2  & 21.9    & 1261.8  \\
FlatVI $\lambda=10$  & 1.2  & 4.2     & 576.9 & 1.7    & 4.8     & 1206.9  & 14.5     & 20.5      & 591.4   & 3.8   & 3.8     & 1342.1  \\ \hline
\end{tabular}}
\end{table*}
%
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/fig_1.pdf} 
    \caption{2D PCA plots of the latent spaces computed by GAE, NB-VAE and FlatVI. Highlighted are initial, intermediate and terminal cell states along the biological trajectory. $\lambda=1$  was fixed for all but the MEF dataset, where $\lambda$ was set to 0.1.}
    \label{fig:latent_representation_vaes}
\end{figure*}

\subsection{Flattening loss}
To model continuous trajectories from discrete data, we would like to perform OT in the latent space of a VAE using a notion of distance that reflects geodesics on the NB statistical manifold. An ideal approach would be to replace straight with geodesic paths in the definition of the OT-CFM objective, ensuring that trajectories in the latent space reflect the data geometry. However, the computation of the geodesic distances for pairs of points entails learning geodesic curves connecting observations minimising \cref{dist} via gradient descent \citep{arvanitidis2022pulling}. This is not feasible for OT-CFM, since the transport matrix requires calculating distances between all pairs of points from batches drawn from the source and the target distributions. 

To ensure that straight latent paths model geodesics along the statistical manifold in an efficient way, we regularise the NB-VAE upfront to induce constant Euclidean local geometry in the latent space before applying OT-CFM. More specifically, if $\mathrm{M}(\mathbf{z})=\mathbb{I}_d$, then the geodesic distance between each pair of latent points is given by the straight line between them. This is achieved by the use of an additional regularisation term to 
the NB-VAE similar to the one implemented for deterministic AEs by \citet{chen2022flat}. Our regularisation is defined as follows:
%
\begin{equation}
\mathcal{L}_\text{flat}=\mathbb{E}_{q(\mathbf{z} \mid \mathbf{x})}\big\lVert \mathrm{M}(\mathbf{z})-\alpha \mathbb{I}_d\big\lVert ^2
\end{equation}
%
with $\mathrm{M}(\mathbf{z})$ calculated by \cref{nb_metric} and where $\alpha$ is a trainable parameter offering some flexibility on the scale of the diagonal constraint. As a result, we enforce a flat geometry in the latent space, where straight-line distances approximate geodesic distances on the statistical manifold. The non-linear decoder $h$ then maps the flat latent space to the curved statistical manifold. The loss of FlatVI, therefore, is
%
\begin{equation}
    \mathcal{L} = \mathcal{L}_\text{ELBO} + \lambda \mathcal{L}_\text{flat} \: ,
\end{equation}
%
where $\lambda$ controls the strength of the flattening regularisation. In practice, we train flows post-hoc on the latent space of the regularised VAE and derive the evolution of gene counts through time by sampling the likelihood model from the decoded parameters. The training procedures for both FlatVI and its combination with OT-CFM are elucidated in \cref{sec: algorithms}.

==> chapters/4_experiments.tex <==
\section{Experiments}
Upon introducing our model, we evaluate FlatVI and its combination with OT-CFM in four biological settings involving trajectories.

\textbf{Baselines \& setup}
We compare the latent space of FlatVI with that of a standard VAE (NB-VAE) trained with an NB decoder \citep{Lopez2018} as representations for continuous OT. Additionally, we evaluate latent OT on the embeddings produced by the Geodesic Autoencoder (GAE) described in 
\citet{mioflow}. The latter is trained on $\log$-normalised gene expression to better accommodate for the lack of a discrete probabilistic decoder. All three approaches are used to derive embeddings of time-resolved gene expression datasets. Subsequently, we use the cell representations to train an OT-CFM model and learn latent trajectories using unpaired batches of observations from consecutive time points. \cref{sec:experimental_setup} provides additional details about the experiments.
%

\textbf{Data}
We evaluate our method for latent trajectory inference on four time-resolved scRNA-seq datasets which have been previously used in trajectory inference studies \citep{eyring2022modeling, Lange2022, tong2023}: 
\begin{inparaenum}[(i)]
\item \textbf{Embryoid body (EB)}. \citet{Moon2019} profile 18,203 differentiating human embryoid cells over five time points, generating four lineages. \item \textbf{Cytomegalovirus infection (CMV)}. \citet{Hein2021} measure 12,919 fibroblasts infected by Cytomegalovirus across seven time points.
\item \textbf{Reprogramming dataset (MEF)}. \citet{Schiebinger2019} explore the reprogramming of mouse embryonic fibroblasts into induced pluripotent stem cells, comprising 165,892 cells across 39 time points and 7 cell states. \item \textbf{Pancreatic endocrinogenesis (Pancreas)}. \citet{BastidasPonce2019} measure 16,206 cells, spanning embryonic days 14.5 to 15.5, revealing multipotent cell differentiation into endocrine and non-endocrine lineages.
\end{inparaenum}
%

\textbf{Evaluation metrics} We analyse our approach considering its representation learning potential as well as its combination with latent OT using the following criteria. 
\begin{inparaenum}[(i)] 
\item \textbf{Degree of flattening}.  We employ the \textit{Variance of the Riemannian metric} (VoR) and the \textit{magnification factor} (MF) metrics following \citet{chen2020learning} and \citet{lee2022regularized} to measure regularisation strength. Briefly, given a metric tensor $\mathrm{M}(\mathbf{z})$, VoR quantifies the uniformity of the Riemannian metric across space by computing the distance between $\mathrm{M}(\mathbf{z})$ and $\Bar{\mathrm{M}}=\mathbb{E}_{\mathbf{z} \sim p_\mathbf{z}}[\mathrm{M}(\mathbf{z})]$. A VoR of 0 indicates constant metric across $\mathcal{Z}$. MF is defined as $\textrm{MF}(\mathbf{z})=\sqrt{\textrm{det} \; \mathrm{M}(\mathbf{z})}$ and reflects the proximity of the metric tensor to the identity $\mathbb{I}_d$. More details are in \cref{app: metric_description}. \item \textbf{Trajectory reconstruction}. When inferring OT trajectories on different representation spaces, we evaluate the quality of the learnt transport map by computing the 2-Wasserstein and mean L$^2$ distances between real and reconstructed latent cells per time point. Additionally, we evaluate the mixing of real and predicted cells in the decoded gene expression space using the nearest-neighbour-based \textit{Density and Coverage} ($D$ \& $C$) metrics \citep{naeem2020reliable}. Density rewards generated samples localised in dense real data regions. Conversely, Coverage quantifies the fraction of real samples whose neighbourhoods contain at least one generated example. \item \textbf{Vector field quality.} We quantify the quality of vector fields learnt by OT in different latent spaces based on their direction consistency within cellular neighbourhoods and their ability to identify cell lineages across time. 
\end{inparaenum}
%
\subsection{Flat latent space properties}
We hypothesise the constraint induced by our regularisation introduces a trade-off between flatness and reconstruction as a function of the hyperparameter $\lambda$. Table~\ref{tab:tradeoff_lik_flatness} depicts the properties of the latent space of FlatVI at increasing levels of regularisation across four datasets. Noticeably, high values of $\lambda$ contribute to a flatter latent space, suggesting our regularisation successfully induces a constant and flat geometry in the VAE bottleneck together with a gradual increase in negative log-likelihood. Setting $\lambda=0$ recovers the NB-VAE model. In practice, a value of $\lambda=1$ is chosen for all datasets but the MEF reprogramming setting, where $\lambda=0.1$ is selected to avoid an excessive penalisation of the gene reconstruction (see \ref{sec:experimental_setup} for more details). Furthermore, we compare the PCA embeddings of our FlatVI's latent space with competing models in Figure~\ref{fig:latent_representation_vaes}. The significantly higher variance explained by the first two principal components demonstrates that our flattening regularisation induces a lower latent space dimensionality, making the information compression more efficient and less noisy. At the same time, the biological structure of the data is preserved or even enhanced compared to competing methods. Biological preservation is particularly evident in the MEF dataset \citep{Schiebinger2019}, where FlatVI induces a clearer separation between initial and terminal states, suggesting a better identification of the cellular dynamics. 

%
\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/fig_2.pdf} % Replace 'example-image' with the filename of your image
    \caption{Prediction of scRNA-seq in time. (\textbf{a})\, Overlap between real and simulated latent samples in the EB dataset. WD indicates the 2-Wasserstein distance between real and generated latent cell representations. (\textbf{b})\, 2D UMAP plots of real and predicted cell counts from the cardiac and neural crest lineages of the EB dataset. Colours indicate the predicted $\log$ gene expression of the reported lineage drivers GYPC and HAND1.}
    \label{fig:rnaseq_simulation}
\end{figure}
%
\subsection{Reconstruction of scRNA-seq trajectories}
% Please add the following required packages to your document preamble:

\begin{table*}[h]
\caption{Comparison of held-out time point reconstruction across models, including the baseline.}\label{tab:leaveout_performance}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc|cccc@{}}
\toprule
                                & \multicolumn{4}{c|}{EB}                                                                                & \multicolumn{4}{c|}{CMV}                                                                               & \multicolumn{4}{c}{MEF}                                                                                \\
\multicolumn{1}{l|}{}           & \multicolumn{2}{c|}{Latent}                                  & \multicolumn{2}{c|}{Decoded}            & \multicolumn{2}{c|}{Latent}                                  & \multicolumn{2}{c|}{Decoded}            & \multicolumn{2}{c|}{Latent}                                  & \multicolumn{2}{c}{Decoded}             \\
\multicolumn{1}{l|}{}           & WD\,(\textdownarrow)                 & \multicolumn{1}{c|}{$L^2$\,(\textdownarrow)}                 & $D$\,(\textuparrow)              & $C$\,(\textuparrow)               & WD\,(\textdownarrow)                 & \multicolumn{1}{c|}{$L^2$\,(\textdownarrow)}                 & $D$\,(\textuparrow)              & $C$\,(\textuparrow)               & WD\,(\textdownarrow)                 & \multicolumn{1}{c|}{$L^2$\,(\textdownarrow)}                 & $D$\,(\textuparrow)              & $C$\,(\textuparrow)               \\ \midrule
\multicolumn{1}{l|}{Baseline}      & 2.69\scriptsize{±0.20}          & \multicolumn{1}{c|}{0.50\scriptsize{±0.08}}          & 0.04\scriptsize{±0.01}          & 0.12\scriptsize{±0.01}          & 2.77\scriptsize{±0.15}          & \multicolumn{1}{c|}{0.55\scriptsize{±0.06}}          & 0.25\scriptsize{±0.06}          & 0.18\scriptsize{±0.03}          & 3.21\scriptsize{±0.16}          & \multicolumn{1}{c|}{0.83\scriptsize{±0.06}}          & 0.12\scriptsize{±0.04}          & 0.07\scriptsize{±0.01}          \\
\multicolumn{1}{l|}{GAE}        & 2.16\scriptsize{±0.14}          & \multicolumn{1}{c|}{0.40\scriptsize{±0.06}}          & 0.05\scriptsize{±0.00}          & 0.02\scriptsize{±0.00}          & 2.10\scriptsize{±0.10}          & \multicolumn{1}{c|}{0.34\scriptsize{±0.04}}          & 0.02\scriptsize{±0.00}          & 0.03\scriptsize{±0.01}          & 2.49\scriptsize{±0.22}          & \multicolumn{1}{c|}{0.57\scriptsize{±0.07}}          & 0.00\scriptsize{±0.00}          & 0.00\scriptsize{±0.00}          \\
\multicolumn{1}{l|}{NB-VAE}     & 2.07\scriptsize{±0.07}          & \multicolumn{1}{c|}{0.30\scriptsize{±0.02}}          & 0.22\scriptsize{±0.03}          & 0.38\scriptsize{±0.03}          & 2.12\scriptsize{±0.08}          & \multicolumn{1}{c|}{\textbf{0.32}\scriptsize{±0.03}} & 1.65\scriptsize{±0.17}          & 0.63\scriptsize{±0.03}          & 2.07\scriptsize{±0.12}          & \multicolumn{1}{c|}{0.40\scriptsize{±0.05}}          & 0.13\scriptsize{±0.02}          & 0.10\scriptsize{±0.01}          \\
\multicolumn{1}{l|}{FlatVI} & \textbf{1.54}\scriptsize{±0.09} & \multicolumn{1}{c|}{\textbf{0.27}\scriptsize{±0.03}} & \textbf{0.31}\scriptsize{±0.05} & \textbf{0.49}\scriptsize{±0.02} & \textbf{1.96}\scriptsize{±0.14} & \multicolumn{1}{c|}{0.37\scriptsize{±0.04}}          & \textbf{3.92}\scriptsize{±0.29} & \textbf{0.85}\scriptsize{±0.03} & \textbf{1.64}\scriptsize{±0.13} & \multicolumn{1}{c|}{\textbf{0.36}\scriptsize{±0.05}} & \textbf{0.16}\scriptsize{±0.04} & \textbf{0.13}\scriptsize{±0.01} \\ \bottomrule
\end{tabular}
}
\end{table*}
% 
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/fig_3.pdf} % Replace 'example-image' with the filename of your image
    \caption{Learning terminal states from OT-CFM's cell velocities in the Pancreas dataset. (\textbf{a})\, Comparison of terminal states found by CellRank using 10-dimensional latent spaces. (\textbf{b})\, Consistency computed for the latent velocities of cells across different latent space dimensionalities.}
    \label{fig:cellrank_experiment}
\end{figure*}
%
Applying OT-CFM to the learnt latent spaces, we can compare simulating latent trajectories from NB-VAE with our FlatVI. Expectedly, modelling latent trajectories with Euclidean cost benefits from a flat statistical manifold, as displayed by the lower 2-Wasserstein distance (WD) between real and simulated latent observations in \cref{fig:rnaseq_simulation}a. Together with latent reconstruction, our approach allows us to gain insight into discrete gene expression counts and study how lineage drivers evolve through time, cf. \cref{fig:rnaseq_simulation}b for examples on the cardiac and neural crest branches of the EB dataset.
% 
To quantify the performance gain of dynamic OT on the flat manifold, we adopt a similar evaluation as \citet{Tong2020TrajectoryNet}. For each dataset, we leave out intermediate time points and train OT-CFM on the remaining cells. The capacity of OT to reconstruct unseen time point $t$ from $t-1$ during inference is an indication of the interpolation abilities of the model along the data manifold. Here, we use such an evaluation paradigm to compare different representation spaces. As a baseline, we calculate the distributional distance between the held-out time point $t$ and the ground truth cells at the previous time point $t-1$. In Table~\ref{tab:leaveout_performance}, we report the reconstruction metrics between true and interpolated latent cells. On almost all datasets and metrics,  trajectories in the flat latent space yield better overall latent time point reconstruction results. This observation is specifically true in the larger MEF reprogramming and EB datasets. Furthermore, the experiments show that our approach yields an overall improvement in the inferred decoded trajectories in the count space, which can be seen by higher Density and Coverage metrics across all evaluated datasets.  
%
\subsection{Latent vector field and lineage mapping}
We hypothesise that dynamic OT with Euclidean cost benefits from being applied to a flat representation space, as the straight path between matched distributions learnt by OT-CFM are optimal paths in an Euclidean space. We evaluate the quality of the cell-specific velocity direction learnt on our flat latent space using the pancreas endocrinogenesis dataset from \citet{BastidasPonce2019}. More specifically, our approach follows the experimental setup introduced by \citet{eyring2022modeling}, where a continuous vector field is learnt by matching cell distributions through time. Using the CellRank model \citep{Lange2022, Weiler2023}, we build random walks on a cell graph based on the directionality of latent velocities learnt by OT-CFM. Walks converge to macrostates representing the end points of the biological process. Figure~\ref{fig:cellrank_experiment}a summarises the number of terminal cell states identified by following the velocity graph. From prior biological knowledge, it is known that the dataset contains six terminal states, which are all identified on the representation computed by our FlatVI. In contrast, on the GAE and NB-VAE's representations, CellRank only captures four and five terminal states, respectively. In Figure~\ref{fig:cellrank_experiment}b, we further evaluate the velocity consistency within neighbourhoods of cells as a function of latent dimensionality. In line with previous results, OT on our flat latent space yields a more consistent velocity field across latent dimensionalities. Additional results comparing our strategy with traditional RNA velocity approaches are reported in \ref{sec: rna_velo}.
%

==> chapters/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We addressed the task of modelling temporal trajectories from unpaired cell distributions by using walks on flat NB manifolds. To achieve this, we introduced FlatVI, a VAE where the pullback metric of the stochastic decoder is regularised to approximate the identity matrix and enforce local Euclidean geometry in the latent space. Our results demonstrate that our flattening procedure not only preserves but also enhances the biological structure in the latent space. By combining this approach with dynamic OT, we observed better prediction outcomes and more consistent vector fields on cellular manifolds. These improvements have practical benefits for central tasks in studying cellular development, such as fate mapping. In future work, we aim to extend the theory to include a broader range of statistical manifolds and single-cell tasks, such as modelling Poisson-distributed chromatin accessibility, estimating latent space distances for batch correction evaluation or enhancing OT-mediated perturbation modelling.



==> sections/neurips_checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}


%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Everything we claim we do in the abstract and introduction we actually do in the following.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss limitations in \S~\ref{app:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide proofs in \S~\ref{app:proofs}, which we refer to from the main paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the model trainings in \S~\ref{app:implementation} and \ref{app:experiments}, and the dataset curation in \S~\ref{app:datasets} and \S~\ref{app:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: {We provide links to multiple implementations of GENOT in  \S~\ref{app:implementation}}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report training details and dataset curation details in \S~\ref{app:datasets}, \S~\ref{app:experiments}, and \S~\ref{app:implementation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report results across multiple runs for all experiments in the main text. For experiments in the appendix we only report results on one run due to limitations in computational resources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only perform single-GPU training, thus we assume there is no limitation to reproduce single experiments / there is no environmental/societal effect due to a single experimental run. The computational burden lies in the large number of different experiments/configurations conducted for this study.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are aware of the NeurIPS Code of Ethics, and to the best of our knowledge- adhere to it. Moreover, we include an impact statement in \S~\ref{app:impact_statement}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include an impact statement in \S~\ref{app:impact_statement}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't release a pretrained model, nor a dataset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite the papers publishing the original data, and provide links to datasets. We don't mention the licenses explicitly, as they are provided by the original publications.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects other than the bone marrow dataset \citep{luecken2021sandbox}. The data is anonymized, and the original publication discusses questions related to research with human individuals.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Only the bone marrow dataset \citep{luecken2021sandbox} stems from human individuals, but the data is anonymized, and the original publication discusses these aspects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

